VIODE: A Simulated Dataset to Address the Challenges of Visual-Inertial Odometry in Dynamic Environments

Dynamic environments such as urban areas are still challenging for popular visual-inertial odometry (VIO) algorithms. Existing datasets typically fail to capture the dynamic nature of these environments, therefore making it difficult to quantitatively evaluate the robustness of existing VIO methods. To address this issue, we propose three contributions: firstly, we provide the VIODE benchmark, a novel dataset recorded from a simulated UAV that navigates in challenging dynamic environments. The unique feature of the VIODE dataset is the systematic introduction of moving objects into the scenes. It includes three environments, each of which is available in four dynamic levels that progressively add moving objects. The dataset contains synchronized stereo images and IMU data, as well as ground-truth trajectories and instance segmentation masks. Secondly, we compare state-of-the-art VIO algorithms on the VIODE dataset and show that they display substantial performance degradation in highly dynamic scenes. Thirdly, we propose a simple extension for visual localization algorithms that relies on semantic information. Our results show that scene semantics are an effective way to mitigate the adverse effects of dynamic objects on VIO algorithms. Finally, we make the VIODE dataset publicly available at https://github.com/kminoda/VIODE.

==> root_final.tex <==

% %% bare_jrnl.tex
% %% V1.4b
% %% 2015/08/26
% %% by Michael Shell
% %% see http://www.michaelshell.org/
% %% for current contact information.
% %%
% %% This is a skeleton file demonstrating the use of IEEEtran.cls
% %% (requires IEEEtran.cls version 1.8b or later) with an IEEE
% %% journal paper.
% %%
% %% Support sites:
% %% http://www.michaelshell.org/tex/ieeetran/
% %% http://www.ctan.org/pkg/ieeetran
% %% and
% %% http://www.ieee.org/

% %%*************************************************************************
% %% Legal Notice:
% %% This code is offered as-is without any warranty either expressed or
% %% implied; without even the implied warranty of MERCHANTABILITY or
% %% FITNESS FOR A PARTICULAR PURPOSE! 
% %% User assumes all risk.
% %% In no event shall the IEEE or any contributor to this code be liable for
% %% any damages or losses, including, but not limited to, incidental,
% %% consequential, or any other damages, resulting from the use or misuse
% %% of any information contained here.
% %%
% %% All comments are the opinions of their respective authors and are not
% %% necessarily endorsed by the IEEE.
% %%
% %% This work is distributed under the LaTeX Project Public License (LPPL)
% %% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
% %% distributed and modified. A copy of the LPPL, version 1.3, is included
% %% in the base LaTeX documentation of all distributions of LaTeX released
% %% 2003/12/01 or later.
% %% Retain all contribution notices and credits.
% %% ** Modified files should be clearly indicated as such, including  **
% %% ** renaming them and changing author support contact information. **
% %%*************************************************************************


% % *** Authors should verify (and, if needed, correct) their LaTeX system  ***
% % *** with the testflow diagnostic prior to trusting their LaTeX platform ***
% % *** with production work. The IEEE's font choices and paper sizes can   ***
% % *** trigger bugs that do not appear when using other class files.       ***                          ***
% % The testflow support page is at:
% % http://www.michaelshell.org/tex/testflow/



% %\documentclass[journal]{IEEEtran}
% \documentclass[letterpaper, 10 pt, journal, twoside]{IEEEtran}
% %
% % If IEEEtran.cls has not been installed into the LaTeX system files,
% % manually specify the path to it like:
% % \documentclass[journal]{../sty/IEEEtran}





% % Some very useful LaTeX packages include:
% % (uncomment the ones you want to load)


% % *** MISC UTILITY PACKAGES ***
% %
% %\usepackage{ifpdf}
% % Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% % compilation based on whether the output is pdf or dvi.
% % usage:
% % \ifpdf
% %   % pdf code
% % \else
% %   % dvi code
% % \fi
% % The latest version of ifpdf.sty can be obtained from:
% % http://www.ctan.org/pkg/ifpdf
% % Also, note that IEEEtran.cls V1.7 and later provides a builtin
% % \ifCLASSINFOpdf conditional that works the same way.
% % When switching from latex to pdflatex and vice-versa, the compiler may
% % have to be run twice to clear warning/error messages.






% % *** CITATION PACKAGES ***
% %
% %\usepackage{cite}
% % cite.sty was written by Donald Arseneau
% % V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% % \cite{} output to follow that of the IEEE. Loading the cite package will
% % result in citation numbers being automatically sorted and properly
% % "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% % cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% % \cite will automatically add leading space, if needed. Use cite.sty's
% % noadjust option (cite.sty V3.8 and later) if you want to turn this off
% % such as if a citation ever needs to be enclosed in parenthesis.
% % cite.sty is already installed on most LaTeX systems. Be sure and use
% % version 5.0 (2009-03-20) and later if using hyperref.sty.
% % The latest version can be obtained at:
% % http://www.ctan.org/pkg/cite
% % The documentation is contained in the cite.sty file itself.






% % *** GRAPHICS RELATED PACKAGES ***
% %
% \ifCLASSINFOpdf
%   % \usepackage[pdftex]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../pdf/}{../jpeg/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
% \else
%   % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
%   % will default to the driver specified in the system graphics.cfg if no
%   % driver is specified.
%   % \usepackage[dvips]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../eps/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.eps}
% \fi
% % graphicx was written by David Carlisle and Sebastian Rahtz. It is
% % required if you want graphics, photos, etc. graphicx.sty is already
% % installed on most LaTeX systems. The latest version and documentation
% % can be obtained at: 
% % http://www.ctan.org/pkg/graphicx
% % Another good source of documentation is "Using Imported Graphics in
% % LaTeX2e" by Keith Reckdahl which can be found at:
% % http://www.ctan.org/pkg/epslatex
% %
% % latex, and pdflatex in dvi mode, support graphics in encapsulated
% % postscript (.eps) format. pdflatex in pdf mode supports graphics
% % in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% % that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% % not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% % which can result in "jaggedy"/blurry rendering of lines and letters as
% % well as large increases in file sizes.
% %
% % You can find documentation about the pdfTeX application at:
% % http://www.tug.org/applications/pdftex





% % *** MATH PACKAGES ***
% %
% %\usepackage{amsmath}
% % A popular package from the American Mathematical Society that provides
% % many useful and powerful commands for dealing with mathematics.
% %
% % Note that the amsmath package sets \interdisplaylinepenalty to 10000
% % thus preventing page breaks from occurring within multiline equations. Use:
% %\interdisplaylinepenalty=2500
% % after loading amsmath to restore such page breaks as IEEEtran.cls normally
% % does. amsmath.sty is already installed on most LaTeX systems. The latest
% % version and documentation can be obtained at:
% % http://www.ctan.org/pkg/amsmath





% % *** SPECIALIZED LIST PACKAGES ***
% %
% %\usepackage{algorithmic}
% % algorithmic.sty was written by Peter Williams and Rogerio Brito.
% % This package provides an algorithmic environment fo describing algorithms.
% % You can use the algorithmic environment in-text or within a figure
% % environment to provide for a floating algorithm. Do NOT use the algorithm
% % floating environment provided by algorithm.sty (by the same authors) or
% % algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% % algorithm float types and packages that provide these will not provide
% % correct IEEE style captions. The latest version and documentation of
% % algorithmic.sty can be obtained at:
% % http://www.ctan.org/pkg/algorithms
% % Also of interest may be the (relatively newer and more customizable)
% % algorithmicx.sty package by Szasz Janos:
% % http://www.ctan.org/pkg/algorithmicx




% % *** ALIGNMENT PACKAGES ***
% %
% %\usepackage{array}
% % Frank Mittelbach's and David Carlisle's array.sty patches and improves
% % the standard LaTeX2e array and tabular environments to provide better
% % appearance and additional user controls. As the default LaTeX2e table
% % generation code is lacking to the point of almost being broken with
% % respect to the quality of the end results, all users are strongly
% % advised to use an enhanced (at the very least that provided by array.sty)
% % set of table tools. array.sty is already installed on most systems. The
% % latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/array


% % IEEEtran contains the IEEEeqnarray family of commands that can be used to
% % generate multiline equations as well as matrices, tables, etc., of high
% % quality.




% % *** SUBFIGURE PACKAGES ***
% %\ifCLASSOPTIONcompsoc
% %  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
% %\else
% %  \usepackage[caption=false,font=footnotesize]{subfig}
% %\fi
% % subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% % for subfigure.sty, the latter of which is no longer maintained and is
% % incompatible with some LaTeX packages including fixltx2e. However,
% % subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% % which will override IEEEtran.cls' handling of captions and this will result
% % in non-IEEE style figure/table captions. To prevent this problem, be sure
% % and invoke subfig.sty's "caption=false" package option (available since
% % subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% % handling of captions.
% % Note that the Computer Society format requires a larger sans serif font
% % than the serif footnote size font used in traditional IEEE formatting
% % and thus the need to invoke different subfig.sty package options depending
% % on whether compsoc mode has been enabled.
% %
% % The latest version and documentation of subfig.sty can be obtained at:
% % http://www.ctan.org/pkg/subfig




% % *** FLOAT PACKAGES ***
% %
% %\usepackage{fixltx2e}
% % fixltx2e, the successor to the earlier fix2col.sty, was written by
% % Frank Mittelbach and David Carlisle. This package corrects a few problems
% % in the LaTeX2e kernel, the most notable of which is that in current
% % LaTeX2e releases, the ordering of single and double column floats is not
% % guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% % single column figure to be placed prior to an earlier double column
% % figure.
% % Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% % corrections already built into the system in which case a warning will
% % be issued if an attempt is made to load fixltx2e.sty as it is no longer
% % needed.
% % The latest version and documentation can be found at:
% % http://www.ctan.org/pkg/fixltx2e


% %\usepackage{stfloats}
% % stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% % the ability to do double column floats at the bottom of the page as well
% % as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% % LaTeX2e). It also provides a command:
% %\fnbelowfloat
% % to enable the placement of footnotes below bottom floats (the standard
% % LaTeX2e kernel puts them above bottom floats). This is an invasive package
% % which rewrites many portions of the LaTeX2e float routines. It may not work
% % with other packages that modify the LaTeX2e float routines. The latest
% % version and documentation can be obtained at:
% % http://www.ctan.org/pkg/stfloats
% % Do not use the stfloats baselinefloat ability as the IEEE does not allow
% % \baselineskip to stretch. Authors submitting work to the IEEE should note
% % that the IEEE rarely uses double column equations and that authors should try
% % to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% % packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% % such ways.
% % Do not attempt to use stfloats with fixltx2e as they are incompatible.
% % Instead, use Morten Hogholm'a dblfloatfix which combines the features
% % of both fixltx2e and stfloats:
% %
% % \usepackage{dblfloatfix}
% % The latest version can be found at:
% % http://www.ctan.org/pkg/dblfloatfix




% %\ifCLASSOPTIONcaptionsoff
% %  \usepackage[nomarkers]{endfloat}
% % \let\MYoriglatexcaption\caption
% % \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
% %\fi
% % endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
% % Axel Sommerfeldt. This package may be useful when used in conjunction with 
% % IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
% % submissions have lists of figures/tables at the end of the paper and that
% % figures/tables without any captions are placed on a page by themselves at
% % the end of the document. If needed, the draftcls IEEEtran class option or
% % \CLASSINPUTbaselinestretch interface can be used to increase the line
% % spacing as well. Be sure and use the nomarkers option of endfloat to
% % prevent endfloat from "marking" where the figures would have been placed
% % in the text. The two hack lines of code above are a slight modification of
% % that suggested by in the endfloat docs (section 8.4.1) to ensure that
% % the full captions always appear in the list of figures/tables - even if
% % the user used the short optional argument of \caption[]{}.
% % IEEE papers do not typically make use of \caption[]'s optional argument,
% % so this should not be an issue. A similar trick can be used to disable
% % captions of packages such as subfig.sty that lack options to turn off
% % the subcaptions:
% % For subfig.sty:
% % \let\MYorigsubfloat\subfloat
% % \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% % However, the above trick will not work if both optional arguments of
% % the \subfloat command are used. Furthermore, there needs to be a
% % description of each subfigure *somewhere* and endfloat does not add
% % subfigure captions to its list of figures. Thus, the best approach is to
% % avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% % and instead reference/explain all the subfigures within the main caption.
% % The latest version of endfloat.sty and its documentation can obtained at:
% % http://www.ctan.org/pkg/endfloat
% %
% % The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% % later in the document, say, to conditionally put the References on a 
% % page by themselves.




% % *** PDF, URL AND HYPERLINK PACKAGES ***
% %
% %\usepackage{url}
% % url.sty was written by Donald Arseneau. It provides better support for
% % handling and breaking URLs. url.sty is already installed on most LaTeX
% % systems. The latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/url
% % Basically, \url{my_url_here}.




% % *** Do not adjust lengths that control margins, column widths, etc. ***
% % *** Do not use packages that alter fonts (such as pslatex).         ***
% % There should be no need to do such things with IEEEtran.cls V1.6 and later.
% % (Unless specifically asked to do so by the journal or conference you plan
% % to submit to, of course. )


% % correct bad hyphenation here
% \hyphenation{op-tical net-works semi-conduc-tor}


% \begin{document}
% %
% % paper title
% % Titles are generally capitalized except for words such as a, an, and, as,
% % at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% % not capitalized unless they are the first or last word of the title.
% % Linebreaks \\ can be used within to get better formatting as desired.
% % Do not put math or special symbols in the title.
% \title{Preparation of Papers for IEEE Robotics and Automation Letters (RA-L)}
% %
% %
% % author names and IEEE memberships
% % note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% % a structure at a ~ so this keeps an author's name from being broken across
% % two lines.
% % use \thanks{} to gain access to the first footnote area
% % a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% % was not built to handle multiple paragraphs
% %

% % \author{Michael~Shell,~\IEEEmembership{Member,~IEEE,}
% %         John~Doe,~\IEEEmembership{Fellow,~OSA,}
% %         and~Jane~Doe,~\IEEEmembership{Life~Fellow,~IEEE}% <-this % stops a space
% % \thanks{M. Shell was with the Department
% % of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta,
% % GA, 30332 USA e-mail: (see http://www.michaelshell.org/contact.html).}% <-this % stops a space
% % \thanks{J. Doe and J. Doe are with Anonymous University.}% <-this % stops a space
% % \thanks{Manuscript received April 19, 2005; revised August 26, 2015.}}
% \author{First A. Author$^{1}$, Second B. Author$^{2}$, and Third C. Author$^{1}$%
% \thanks{Manuscript received: Month, Day, Year; Revised Month, Day, Year; Accepted Month, Day, Year.}%Use only for final RAL version
% \thanks{This paper was recommended for publication by Editor FirstName A. EditorName upon evaluation of the Associate Editor and Reviewers' comments.
% This work was supported by (organizations/grants which supported the work.)} %Use only for final RAL version
% \thanks{$^{1}$First Author and Third Author are with School of Engineering, Robotics Department, University of Somewhere, Someland
%         {\tt\footnotesize first.author@papercept.net}}%
% \thanks{$^{2} $SecondAuthor is with School of Engineering, Automation Department, University of Anywhere, Anyland
%         {\tt\footnotesizel second.author@papercept.net}}%
% \thanks{Digital Object Identifier (DOI): see top of this page.}
% }
% % note the % following the last \IEEEmembership and also \thanks - 
% % these prevent an unwanted space from occurring between the last author name
% % and the end of the author line. i.e., if you had this:
% % 
% % \author{....lastname \thanks{...} \thanks{...} }
% %                     ^------------^------------^----Do not want these spaces!
% %
% % a space would be appended to the last name and could cause every name on that
% % line to be shifted left slightly. This is one of those "LaTeX things". For
% % instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% % "AB" then you have to do: "\textbf{A}\textbf{B}"
% % \thanks is no different in this regard, so shield the last } of each \thanks
% % that ends a line with a % and do not let a space in before the next \thanks.
% % Spaces after \IEEEmembership other than the last one are OK (and needed) as
% % you are supposed to have spaces between the names. For what it is worth,
% % this is a minor point as most people would not even notice if the said evil
% % space somehow managed to creep in.



% % The paper headers
% %\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
% %{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
% \markboth{IEEE Robotics and Automation Letters. Preprint Version. Accepted Month, Year}
% {FirstAuthorSurname \MakeLowercase{\textit{et al.}}: ShortTitle} 

% % The only time the second header will appear is for the odd numbered pages
% % after the title page when using the twoside option.
% % 
% % *** Note that you probably will NOT want to include the author's ***
% % *** name in the headers of peer review papers.                   ***
% % You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% % you desire.




% % If you want to put a publisher's ID mark on the page you can do it like
% % this:
% %\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% % Remember, if you use this you must call \IEEEpubidadjcol in the second
% % column for its text to clear the IEEEpubid mark.



% % use for special paper notices
% %\IEEEspecialpapernotice{(Invited Paper)}




% % make the title area
% \maketitle

% % As a general rule, do not put math, special symbols or citations
% % in the abstract or keywords.
% \begin{abstract}
% These instructions give you guidelines for preparing papers for IEEE Transactions and Journals. Use this document as a sample output. Paper titles should be written in uppercase and lowercase letters, not all uppercase. Avoid writing long formulas with subscripts in the title; short formulas that identify the elements are fine (e.g., "Nd?Fe?B"). Full names of authors are preferred in the author field, but are not required. Put a space between authors�f initials. Define all symbols used in the abstract. Do not cite references in the abstract. Do not delete the blank line immediately above the abstract; it sets the footnote at the bottom of this column.
% \end{abstract}

% % Note that keywords are not normally used for peerreview papers.
% % \begin{IEEEkeywords}
% % IEEE, IEEEtran, journal, \LaTeX, paper, template.
% % \end{IEEEkeywords}
% \begin{IEEEkeywords}
% List of keywords (from the RA Letters keyword list)
% \end{IEEEkeywords}





% % For peer review papers, you can put extra information on the cover
% % page as needed:
% % \ifCLASSOPTIONpeerreview
% % \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% % \fi
% %
% % For peerreview papers, this IEEEtran command inserts a page break and
% % creates the second title. It will be ignored for other modes.
% \IEEEpeerreviewmaketitle



% \section{Introduction}
% % The very first letter is a 2 line initial drop letter followed
% % by the rest of the first word in caps.
% % 
% % form to use if the first word consists of a single letter:
% % \IEEEPARstart{A}{demo} file is ....
% % 
% % form to use if you need the single drop letter followed by
% % normal text (unknown if ever used by the IEEE):
% % \IEEEPARstart{A}{}demo file is ....
% % 
% % Some journals put the first two words in caps:
% % \IEEEPARstart{T}{his demo} file is ....
% % 
% % Here we have the typical use of a "T" for an initial drop letter
% % and "HIS" in caps to complete the first word.
% % \IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
% % for IEEE journal papers produced under \LaTeX\ using
% % IEEEtran.cls version 1.8b and later.
% % You must have at least 2 lines in the paragraph with the drop letter
% % (should never be an issue)
% \IEEEPARstart{T}{his} is the first sentence of my Introduction.
% I wish you the best of success.
% This is the second sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.
% This is the following sentence of my Introduction.

% % \hfill mds
% %  
% % \hfill August 26, 2015

% \section{Next Section}
% \subsection{Subsection Heading Here}
% Subsection text here.
% Subsection text here.
% Subsection text here.
% Subsection text here.
% Subsection text here.
% Subsection text here.
% Subsection text here.
% Subsection text here.
% Subsection text here.

% % needed in second column of first page if using \IEEEpubid
% %\IEEEpubidadjcol

% \subsubsection{Subsubsection Heading Here}
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.
% Subsubsection text here.

% \subsubsection{Next Subsubsection Heading Here}
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.


% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.


% \section{Next Section}
% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.


% \section{Next Section}
% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% \subsubsection{Next Subsubsection Heading Here}
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.

% \subsubsection{Next Subsubsection Heading Here}
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.

% \subsubsection{Next Subsubsection Heading Here}
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.



% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.


% \section{Next Section}
% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% \subsubsection{Next Subsubsection Heading Here}
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.


% \subsubsection{Next Subsubsection Heading Here}
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.


% \subsubsection{Next Subsubsection Heading Here}
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.
% Next subsubsection text here.



% \section{Next Section}
% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% \subsection{Next Subsection Heading Here}
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.
% Next subsection text here.

% % An example of a floating figure using the graphicx package.
% % Note that \label must occur AFTER (or within) \caption.
% % For figures, \caption should occur after the \includegraphics.
% % Note that IEEEtran v1.7 and later has special internal code that
% % is designed to preserve the operation of \label within \caption
% % even when the captionsoff option is in effect. However, because
% % of issues like this, it may be the safest practice to put all your
% % \label just after \caption rather than within \caption{}.
% %
% % Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% % option should be used if it is desired that the figures are to be
% % displayed while in draft mode.
% %
% %\begin{figure}[!t]
% %\centering
% %\includegraphics[width=2.5in]{myfigure}
% % where an .eps filename suffix will be assumed under latex, 
% % and a .pdf suffix will be assumed for pdflatex; or what has been declared
% % via \DeclareGraphicsExtensions.
% %\caption{Simulation results for the network.}
% %\label{fig_sim}
% %\end{figure}

% % Note that the IEEE typically puts floats only at the top, even when this
% % results in a large percentage of a column being occupied by floats.


% % An example of a double column floating figure using two subfigures.
% % (The subfig.sty package must be loaded for this to work.)
% % The subfigure \label commands are set within each subfloat command,
% % and the \label for the overall figure must come after \caption.
% % \hfil is used as a separator to get equal spacing.
% % Watch out that the combined width of all the subfigures on a 
% % line do not exceed the text width or a line break will occur.
% %
% %\begin{figure*}[!t]
% %\centering
% %\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
% %\label{fig_first_case}}
% %\hfil
% %\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
% %\label{fig_second_case}}
% %\caption{Simulation results for the network.}
% %\label{fig_sim}
% %\end{figure*}
% %
% % Note that often IEEE papers with subfigures do not employ subfigure
% % captions (using the optional argument to \subfloat[]), but instead will
% % reference/describe all of them (a), (b), etc., within the main caption.
% % Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% % labels, the optional argument to \subfloat must be present. If a
% % subcaption is not desired, just leave its contents blank,
% % e.g., \subfloat[].


% % An example of a floating table. Note that, for IEEE style tables, the
% % \caption command should come BEFORE the table and, given that table
% % captions serve much like titles, are usually capitalized except for words
% % such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% % and up, which are usually not capitalized unless they are the first or
% % last word of the caption. Table text will default to \footnotesize as
% % the IEEE normally uses this smaller font for tables.
% % The \label must come after \caption as always.
% %
% %\begin{table}[!t]
% %% increase table row spacing, adjust to taste
% %\renewcommand{\arraystretch}{1.3}
% % if using array.sty, it might be a good idea to tweak the value of
% % \extrarowheight as needed to properly center the text within the cells
% %\caption{An Example of a Table}
% %\label{table_example}
% %\centering
% %% Some packages, such as MDW tools, offer better commands for making tables
% %% than the plain LaTeX2e tabular which is used here.
% %\begin{tabular}{|c||c|}
% %\hline
% %One & Two\\
% %\hline
% %Three & Four\\
% %\hline
% %\end{tabular}
% %\end{table}


% % Note that the IEEE does not put floats in the very first column
% % - or typically anywhere on the first page for that matter. Also,
% % in-text middle ("here") positioning is typically not used, but it
% % is allowed and encouraged for Computer Society conferences (but
% % not Computer Society journals). Most IEEE journals/conferences use
% % top floats exclusively. 
% % Note that, LaTeX2e, unlike IEEE journals/conferences, places
% % footnotes above bottom floats. This can be corrected via the
% % \fnbelowfloat command of the stfloats package.




% \section{Conclusion}
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.
% The conclusion goes here.





% % if have a single appendix:
% %\appendix[Proof of the Zonklar Equations]
% % or
% %\appendix  % for no appendix heading
% % do not use \section anymore after \appendix, only \section*
% % is possibly needed

% % use appendices with more than one appendix
% % then use \section to start each appendix
% % you must declare a \section before using any
% % \subsection or using \label (\appendices by itself
% % starts a section numbered zero.)
% %


% \appendices
% \section{Proof of the First Zonklar Equation}
% Appendix one text goes here.

% % you can choose not to have a title for an appendix
% % if you want by leaving the argument blank
% \section{}
% Appendix two text goes here.


% % use section* for acknowledgment
% \section*{Acknowledgment}


% The authors would like to thank...


% % Can use something like this to put references on a page
% % by themselves when using endfloat and the captionsoff option.
% \ifCLASSOPTIONcaptionsoff
%   \newpage
% \fi



% % trigger a \newpage just before the given reference
% % number - used to balance the columns on the last page
% % adjust value as needed - may need to be readjusted if
% % the document is modified later
% %\IEEEtriggeratref{8}
% % The "triggered" command can be changed if desired:
% %\IEEEtriggercmd{\enlargethispage{-5in}}

% % references section

% % can use a bibliography generated by BibTeX as a .bbl file
% % BibTeX documentation can be easily obtained at:
% % http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% % The IEEEtran BibTeX style support page is at:
% % http://www.michaelshell.org/tex/ieeetran/bibtex/
% %\bibliographystyle{IEEEtran}
% % argument is your BibTeX string definitions and bibliography database(s)
% %\bibliography{IEEEabrv,../bib/paper}
% %
% % <OR> manually copy in the resultant .bbl file
% % set second argument of \begin to the number of references
% % (used to reserve space for the reference number labels box)
% \begin{thebibliography}{1}

% \bibitem{IEEEhowto:kopka}
% H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%   0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

% \end{thebibliography}

% % biography section
% % 
% % If you have an EPS/PDF photo (graphicx package needed) extra braces are
% % needed around the contents of the optional argument to biography to prevent
% % the LaTeX parser from getting confused when it sees the complicated
% % \includegraphics command within an optional argument. (You could create
% % your own custom macro containing the \includegraphics command to make things
% % simpler here.)
% %\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% % or if you just want to reserve a space for a photo:

% \begin{IEEEbiography}{Michael Shell}
% Biography text here.
% \end{IEEEbiography}

% % if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% % insert where needed to balance the two columns on the last page with
% % biographies
% %\newpage

% \begin{IEEEbiographynophoto}{Jane Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% % You can push biographies down or up by placing
% % a \vfill before or after them. The appropriate
% % use of \vfill depends on what kind of text is
% % on the last page and whether or not the columns
% % are being equalized.

% %\vfill

% % Can be used to pull up biographies so that the bottom of the last one
% % is flush with the other column.
% %\enlargethispage{-5in}



% % that's all folks
% \end{document}




==> root_original.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %2345678901234567890123456789012345678901234567890123456789012345678901234567890
% %        1         2         3         4         5         6         7         8

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}  % Comment this line out if you need a4paper

% %\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4 paper

% \IEEEoverridecommandlockouts                              % This command is only needed if 
%                                                           % you want to use the \thanks command

% \overrideIEEEmargins                                      % Needed to meet printer requirements.

% %In case you encounter the following error:
% %Error 1010 The PDF file may be corrupt (unable to open PDF file) OR
% %Error 1000 An error occurred while parsing a contents stream. Unable to analyze the PDF file.
% %This is a known problem with pdfLaTeX conversion filter. The file cannot be opened with acrobat reader
% %Please use one of the alternatives below to circumvent this error by uncommenting one or the other
% %\pdfobjcompresslevel=0
% %\pdfminorversion=4

% % See the \addtolength command later in the file to balance the column lengths
% % on the last page of the document

% % The following packages can be found on http:\\www.ctan.org
% %\usepackage{graphics} % for pdf, bitmapped graphics files
% %\usepackage{epsfig} % for postscript graphics files
% %\usepackage{mathptmx} % assumes new font selection scheme installed
% %\usepackage{times} % assumes new font selection scheme installed
% %\usepackage{amsmath} % assumes amsmath package installed
% %\usepackage{amssymb}  % assumes amsmath package installed

% \title{\LARGE \bf
% Preparation of Papers for IEEE Sponsored Conferences \& Symposia*
% }


% \author{Albert Author$^{1}$ and Bernard D. Researcher$^{2}$% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
% \thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
%         University of Twente, 7500 AE Enschede, The Netherlands
%         {\tt\small albert.author@papercept.net}}%
% \thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
%         Dayton, OH 45435, USA
%         {\tt\small b.d.researcher@ieee.org}}%
% }


% \begin{document}



% \maketitle
% \thispagestyle{empty}
% \pagestyle{empty}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract}

% This electronic document is a �live� template. The various components of your paper [title, text, heads, etc.] are already defined on the style sheet, as illustrated by the portions given in this document.

% \end{abstract}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{INTRODUCTION}

% This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

% \section{PROCEDURE FOR PAPER SUBMISSION}

% \subsection{Selecting a Template (Heading 2)}

% First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
% It may be used for A4 paper size if the paper size setting is suitably modified.

% \subsection{Maintaining the Integrity of the Specifications}

% The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

% \section{MATH}

% Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

% Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

% \subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

% \subsection{Units}

% \begin{itemize}

% \item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as �3.5-inch disk drive�.
% \item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
% \item Do not mix complete spellings and abbreviations of units: �Wb/m2� or �webers per square meter�, not �webers/m2�.  Spell out units when they appear in text: �. . . a few henries�, not �. . . a few H�.
% \item Use a zero before decimal points: �0.25�, not �.25�. Use �cm3�, not �cc�. (bullet list)

% \end{itemize}


% \subsection{Equations}

% The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

% $$
% \alpha + \beta = \chi \eqno{(1)}
% $$

% Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use �(1)�, not �Eq. (1)� or �equation (1)�, except at the beginning of a sentence: �Equation (1) is . . .�

% \subsection{Some Common Mistakes}
% \begin{itemize}


% \item The word �data� is plural, not singular.
% \item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter �o�.
% \item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
% \item A graph within a graph is an �inset�, not an �insert�. The word alternatively is preferred to the word �alternately� (unless you really mean something that alternates).
% \item Do not use the word �essentially� to mean �approximately� or �effectively�.
% \item In your paper title, if the words �that uses� can accurately replace the word �using�, capitalize the �u�; if not, keep using lower-cased.
% \item Be aware of the different meanings of the homophones �affect� and �effect�, �complement� and �compliment�, �discreet� and �discrete�, �principal� and �principle�.
% \item Do not confuse �imply� and �infer�.
% \item The prefix �non� is not a word; it should be joined to the word it modifies, usually without a hyphen.
% \item There is no period after the �et� in the Latin abbreviation �et al.�.
% \item The abbreviation �i.e.� means �that is�, and the abbreviation �e.g.� means �for example�.

% \end{itemize}


% \section{USING THE TEMPLATE}

% Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

% It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

% \subsection{Headings, etc}

% Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named �Heading 1�, �Heading 2�, �Heading 3�, and �Heading 4� are prescribed.

% \subsection{Figures and Tables}

% Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation �Fig. 1�, even at the beginning of a sentence.

% \begin{table}[h]
% \caption{An Example of a Table}
% \label{table_example}
% \begin{center}
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}


%   \begin{figure}[thpb]
%       \centering
%       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% }}
%       %\includegraphics[scale=1.0]{figurefile}
%       \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{figurelabel}
%   \end{figure}
   

% Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity �Magnetization�, or �Magnetization, M�, not just �M�. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write �Magnetization (A/m)� or �Magnetization {A[m(1)]}�, not just �A/m�. Do not label axes with a ratio of quantities and units. For example, write �Temperature (K)�, not �Temperature/K.�

% \section{CONCLUSIONS}

% A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{APPENDIX}

% Appendixes should appear before the acknowledgment.

% \section*{ACKNOWLEDGMENT}

% The preferred spelling of the word �acknowledgment� in America is without an �e� after the �g�. Avoid the stilted expression, �One of us (R. B. G.) thanks . . .�  Instead, try �R. B. G. thanks�. Put sponsor acknowledgments in the unnumbered footnote on the first page.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



% \begin{thebibliography}{99}

% \bibitem{c1} G. O. Young, �Synthetic structure of industrial plastics (Book style with paper title and editor),� 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15�64.
% \bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123�135.
% \bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
% \bibitem{c4} B. Smith, �An approach to graphs of linear forms (Unpublished work style),� unpublished.
% \bibitem{c5} E. H. Miller, �A note on reflector arrays (Periodical style�Accepted for publication),� IEEE Trans. Antennas Propagat., to be publised.
% \bibitem{c6} J. Wang, �Fundamentals of erbium-doped fiber amplifiers arrays (Periodical style�Submitted for publication),� IEEE J. Quantum Electron., submitted for publication.
% \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% \bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, �Electron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),� IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740�741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
% \bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
% \bibitem{c10} J. U. Duncombe, �Infrared navigation�Part I: An assessment of feasibility (Periodical style),� IEEE Trans. Electron Devices, vol. ED-11, pp. 34�39, Jan. 1959.
% \bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, �A clustering technique for digital communications channel equalization using radial basis function networks,� IEEE Trans. Neural Networks, vol. 4, pp. 570�578, July 1993.
% \bibitem{c12} R. W. Lucky, �Automatic equalization for digital communication,� Bell Syst. Tech. J., vol. 44, no. 4, pp. 547�588, Apr. 1965.
% \bibitem{c13} S. P. Bingulac, �On the compatibility of adaptive controllers (Published Conference Proceedings style),� in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8�16.
% \bibitem{c14} G. R. Faulhaber, �Design of service systems with priority reservation,� in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3�8.
% \bibitem{c15} W. D. Doyle, �Magnetization reversal in films with biaxial anisotropy,� in 1987 Proc. INTERMAG Conf., pp. 2.2-1�2.2-6.
% \bibitem{c16} G. W. Juette and L. E. Zeffanella, �Radio noise currents n short sections on bundle conductors (Presented Conference Paper style),� presented at the IEEE Summer power Meeting, Dallas, TX, June 22�27, 1990, Paper 90 SM 690-0 PWRS.
% \bibitem{c17} J. G. Kreifeldt, �An analysis of surface-detected EMG as an amplitude-modulated noise,� presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% \bibitem{c18} J. Williams, �Narrow-band analyzer (Thesis or Dissertation style),� Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% \bibitem{c19} N. Kawasaki, �Parametric study of thermal and chemical nonequilibrium nozzle flow,� M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% \bibitem{c20} J. P. Wilkinson, �Nonlinear resonant circuit devices (Patent style),� U.S. Patent 3 624 12, July 16, 1990. 






% \end{thebibliography}




% \end{document}

